A survey on deep learning approaches for data integration in autonomous driving system

The perception module of self-driving vehicles relies on a multi-sensor system to understand its environment. Recent advancements in deep learning have led to the rapid development of approaches that integrate multi-sensory measurements to enhance perception capabilities. This paper surveys the latest deep learning integration techniques applied to the perception module in autonomous driving systems, categorizing integration approaches based on "what, how, and when to integrate". A new taxonomy of integration is proposed, based on three dimensions: multi-view, multi-modality, and multi-frame. The integration operations and their pros and cons are summarized, providing new insights into the properties of an "ideal" data integration approach that can alleviate the limitations of existing methods. After reviewing hundreds of relevant papers, this survey concludes with a discussion of the key features of an optimal data integration approach.

==> sections/custom_defined_command.tex <==
\newcommand{\secref}[1]{Section~#1}
\newcommand{\ie}{i.e.}

==> sections/outline.tex <==
\section{Outline}

\subsection{Introduction}
\subsubsection{Background}
\begin{itemize}
    
    \item Research fields that encounter data integration
    
    \item Significance of data integration in ADS perception

    \item Sensor data integration categories: by data type (modality), by integration levels, by scenarios/tasks

    \item Sensor data integration methods (higher level): traditional methods, deep learning methods

\end{itemize}

\subsubsection{Definition of related concepts in existing literature and clarification}
A brief review of related concepts – what are they and how they overlap with/distinguish from each other:
\begin{itemize}
    \item multi-source, multi-sensor, multi-modal, multi-view
    \item data fusion, data integration, data aggregation, sensor fusion, information fusion
\end{itemize}

\subsubsection{Purpose and boundaries of our survey}
\begin{itemize}
    \item existing data integration surveys focus on specific applications or classiﬁcations
    \item Boundaries: Only sensor data. Focus on data integration process. Up to 5 years (2017 to 2022). Related to deep learning/AI methods.
\end{itemize}

\subsection{Sensors and Properties}
\begin{itemize}
    \item Intro of typical sensors (camera, lidar, radar, ultrasound, IMU, GPS, communication sensors) equipped by autonomous driving vehicles
    \begin{itemize}
        \item a summary (a table) of each sensor’s characteristics (such as data format), advantages, disadvantages, coverage range/maximum distances
    \end{itemize}
\end{itemize}

\subsection{Deep learning approaches for data integration}
\subsubsection{Data Integration categories}
\begin{itemize}
    \item Overview of basic theories of deep learning
    \item Two categories in sensor data integration: Intra-sensor integration, Inter-/cross-sensor integration
\end{itemize}

\includegraphics[width=\linewidth]{figs/sensor_relationship.png}

\subsubsection{Intra-sensor integration: integrates with itself}
\begin{itemize}
    \item camera data integration: spatial -- multi-view/stereo, temporal -- image sequence/video
    \item lidar data integration: (spatial and temporal) denser point cloud
\end{itemize}

\subsubsection{Inter-/cross-sensor integration: multi-source}
\begin{itemize}
    \item camera + lidar, camera + radar, camera + imu, radar + lidar, camera + lidar + radar, camera + lidar + imu, gnss + lidar + imu (+ dmi), communication sensors (V2X)
\end{itemize}

\subsubsection{Existing challenges}
\begin{itemize}
    \item concept of static and dynamic data fusion
    \item limitation of static fusion and necessity of dynamic fusion
\end{itemize}

\subsection{Integration output representation}
A summary of output format after data integration.
\begin{itemize}
    \item concatenated tensor
    \item relation graph
    \item \dots
\end{itemize}

\subsection{Case study}
\subsubsection{ADS application}
\begin{itemize}
    \item input -- data integration -- output process
    \item possible comparisons and insights
\end{itemize}
\subsubsection{Smart-home application}
\subsubsection{Warehousing logistics}
\subsubsection{Supermarket}

\subsection{Conclusion and discussion}
\begin{itemize}
    \item Current focuses in data integration in ADS and future directions
    \item A vision of boarder inter-sensor integration (in a sense of V2X, etc.)
    \item Dynamic fusion
\end{itemize}







==> sections/outline_detailed.tex <==
\section{Outline}

\subsection{Introduction}
\subsubsection{Background}
\begin{itemize}
    \item General overview on data integration
    \begin{itemize}
        \item Which research field encounters data integration?
        \item How many kinds of data integration exists?
        \item Our focus and the progress of our focus
    \end{itemize}
    
    \item Research fields that encounter data integration
    
    
    \item Perception in autonomous driving system. 
    \begin{itemize}
        \item ADS architecture and modules.
        \item Common tasks in perception module: Environment perception and localization. 
        \begin{itemize}
            \item Environment perception: detecting various moving and static obstacles (e.g., vehicles, pedestrians, etc.), and collecting various information on the road (such as drivable areas, road markings, traffic signs, traffic lights, etc.). Sensors for these tasks mainly include cameras, lidars, mmv-radars, etc.
            \item Localization: positioning and localization determines the location of the vehicle in the environment based on the information obtained from environment perception, which always requires high-precision maps, as well as IMU and GPS.
        \end{itemize}
%        \textcolor{purple}{Question here: does our survey include both or only the environment perception?}
        \item Target of the perception module: e.g., to perceive, recognize, understand the scene and the road environment within a certain range of the ego car. In-and-Out of the perception module: sensor data inputs, traffic-related elements/features (both static and dynamic) and location outputs.
        \item The performance of the perception module may directly determines the performance of the downstream modules (prediction, planning, control) and the safety of the vehicle. 
    \end{itemize}
    
    \item Significance of sensor integration in perception
    \begin{itemize}
        \item limitations (temporal and spatial coverage) and uncertainties of a single sensor -- extend coverage and decrease uncertainty
        \begin{itemize}
            \item e.g., cameras have high resolution with color information, while it can not provide depth information or work well in scenarios with low-visibility
            \item e.g., LiDAR may have depth estimation and wide range of view, yet it is vulnerable in bad weathers. 
            \item e.g., while in-vehicle sensors may cooperate to achieve a more comprehensive perception with intra- and inter-sensor integration, a boarder ''inter-sensor'' integration, i.e., V2X (vehicle to connect to everything in the traffic scenario) sensor integration may further extend the scope of the perception of ADS. 
        \end{itemize}
        \item deprivation, if a sensor stops working or can not function well -- increase reliability and robustness
        \item imprecision -- improve resolution and precision
        \item \dots
    \end{itemize}
    
    \item Sensor data integration categories: 
    \begin{itemize}
        \item by data type (modality, e.g., lidar-lidar fusion, camera-lidar fusion)
        \item by integration levels (raw-data/pixel-level, feature-level, object-level, decision-level)
        \item by scenarios/tasks (e.g., object detection, semantic segmentation)
    \end{itemize}
    
    \item Sensor data integration methods (higher level):
    \begin{itemize}
        \item traditional methods (some examples – a brief review)
        \item deep learning methods developed in recent years (a brief review)
    \end{itemize}
\end{itemize}

\subsubsection{Definition of related concepts in existing literature and clarification}
A brief review of related concepts – what are they and how they overlap with/distinguish from each other:
\begin{itemize}
    \item multi-source, multi-sensor, multi-modal, multi-view
    \item data fusion, data integration, data aggregation, sensor fusion, information fusion
\end{itemize}

\subsubsection{Purpose and boundaries of our survey}
\begin{itemize}
    \item Purposes
    \begin{itemize}
        \item deep learning approaches of multi-sensor data integration to enhance the usage of ADS (to be modified)
        \item summarize and present the integration methods by different combination of data types.
        \item \dots
    \end{itemize}
    \item Boundaries
    \begin{itemize}
%        \item \textcolor{purple}{Only environment perception, not localization}
        \item Only sensor data (other data such as radio or text data is not discussed)
        \item Closely related to data integration (technologies that are not related to data integration are not discussed)
        \item Up to 5 years (the most up-to-date works – 2017 to 2022)
        \item More focus on deep learning/AI methods
        \item \dots
    \end{itemize}
\end{itemize}

\subsection{Sensors and Properties}
\begin{itemize}
    \item (Brief intro) Typical autonomous driving vehicles may equip with various kinds of sensors, including: cameras, mmw-radar, LiDAR, ultrasonic,
%    \textcolor{purple}{the global positioning system (GPS)},
    inertial measurement unit (IMU), communication (V2V, V2I, V2X, etc.) sensors.
    \item The characteristics, advantages, and disadvantages of these sensors
    \begin{itemize}
        \item Describe how each sensor works and corresponding characteristics, advantages and disadvantages in subsections.
        \item A summary (a table) of each sensor’s characteristics (such as data format), advantages, disadvantages, coverage range/maximum distances
    \end{itemize}
\end{itemize}

\subsection{Deep learning approaches for data integration in ADS}
\subsubsection{Data Integration categories}
\begin{itemize}
    \item The explosion of this round of autonomous driving technology is largely due to the breakthroughs made by deep learning in the field of computer vision. 
    \item Overview of basic theories of deep learning

    \item Sensor integration can broadly be divided into two categories:
    \begin{itemize}
        \item Intra-sensor integration: sensor integrates with itself -- e.g., integrating temporally or spatially
        \begin{itemize}
            \item camera image integration: e.g., multi-view (direction) camera image integration
            \item lidar dense data integration -- e.g., LiDAR-SLAM
            \item \dots
        \end{itemize}
        
        \item Inter-/cross-sensor integration: multi-modality, different types of sensors' data integrate together
        \begin{itemize}
            \item camera + lidar 
            \item camera + IMU (VIO)
            \item \dots
            \item V2X (car as a whole sensor)
        \end{itemize}
    \end{itemize}

    \item In the following subsections, we will discuss deep learning technologies, how they developed, advantages and disadvantages, when tackling data integration problem in each of the aforementioned integration types.
    
\end{itemize}

\subsubsection{Intra-sensor integration}

\subsubsection{Inter-sensor integration}




\subsection{Industry}
We have talked about various components.
    \subsubsection{The leading companies}
    \subsubsection{Technical choices of leading companies}
    \subsubsection{Comparison of the SOTA products}
    \subsubsection{Weakness and vision}






==> sections/paper_searching_keywords.tex <==
\section{Paper Searching Keywords (and combinations)}

\begin{itemize}
    \item Task
    \begin{itemize}
        \item perception
        \item detection
        \item segmentation
        \item prediction
        \item depth estimation/ normal estimation
        \item tracking
        \item SLAM
        \item 3D reconstruction / dense reconstruction/ multi view stereo/ mapping
    \end{itemize}
    \item Input
    \begin{itemize}
        \item Abstract
        \begin{itemize}
            \item multi-source/multi-modal/modality
            \item multi-sensor 
            \item multi-view
            \item cross-image
        \end{itemize}
        \item Detail
            \begin{itemize}
                \item camera + lidar
                \item camera + radar
                \item camera + imu
                \item binocular
                \item monocular video
                \item radar + lidar
                \item camera + lidar + imu
                \item camera + lidar + radar
                \item gnss + lidar + imu 
                \item gnss + lidar + imu + dmi 
                \item communication sensors/ 5G V2X
            \end{itemize}
    \end{itemize}
    \item Process
    \begin{itemize}
        \item  data fusion, data integration, data aggregation, sensor fusion, information fusion, (sensor alignment, feature alignment)
        \item deep learning
    \end{itemize}
    \item Synonym
    \begin{itemize}
        \item camera/vision/monocular/stereo/image/optical
        \item lidar/laser
        \item radar/mmwave (MMW) radar
        \item IMU/DMI/odometry/speedometry/INS
        \item GNSS/GPS
        \item V2X, V2V, V2N, V2I
    \end{itemize}
\end{itemize}

\subsection{Keywords Combinations}
\begin{itemize}
    \item Big picture
    \begin{itemize}
        \item \$task\$, \$sensors\$, perception, autonomous driving (system)/ ADS
        \item \$input-abstract\$, \$process\$, smart-home, smart-warehousing, smart-supermarket
    \end{itemize}
    \item Specific domains
    \begin{itemize}
        \item \{(object/ car/ pedestrian/ lane line) detection/ recognition\} + \$Process\$
        \item \{(semantic/ instance/ panoramic) segmentation/ pixel-wise classification\} + \$Process\$
        \item \{(object/ car/ pedestrian) tracking/ re-identification/ re-ID\} + \$Process\$
        \item \{SLAM/reconstruction/depth/localization/multi-view/stereo/monocular/binocular\} + \$Process\$
    \end{itemize}
\end{itemize}

\subsection{Paper organization}
Put all papers \href{https://onebox.huawei.com/#eSpaceGroupFile/1/397/7741511}{here}. Please name files as '[year] title' and replace all illegal characters, e.g., ':', with '-'. For example, given a paper published in 2016 named 'Multi-sensor fusion in body sensor networks: State-of-the-art and research challenges', the file name should be '[2016] Multi-sensor fusion in body sensor networks- State-of-the-art and challenges.pdf'.






